Exploiting homogeneity for the optimal control of discrete-time systems: application to value iteration

To investigate solutions of (near-)optimal control problems, we extend and exploit a notion of homogeneity recently proposed in the literature for discrete-time systems. Assuming the plant dynamics is homogeneous, we first derive a scaling property of its solutions along rays provided the sequence of inputs is suitably modified. We then consider homogeneous cost functions and reveal how the optimal value function scales along rays. This result can be used to construct (near-)optimal inputs on the whole state space by only solving the original problem on a given compact manifold of a smaller dimension. Compared to the related works of the literature, we impose no conditions on the homogeneity degrees. We demonstrate the strength of this new result by presenting a new approximate scheme for value iteration, which is one of the pillars of dynamic programming. The new algorithm provides guaranteed lower and upper estimates of the true value function at any iteration and has several appealing features in terms of reduced computation. A numerical case study is provided to illustrate the proposed algorithm.

==> extra.tex <==
 \newpage 

 \appendix
 \mathieu{To do:} %XXX
 \begin{itemize}
     \item Fix number of pages   - argue for removal of section ensuring      \item explicit MPC note
     \item 
     \item Use a higher resolution for classical VI and lower for VI hom
     \item To check Prop 2 and lemma 3
     \item make a sweep for input sequence length.
 
\end{itemize}

\newpage\onecolumn\doublespacing
%%%%%%%%%%%%%%%%%%

\section{Comments}
%%%%%%%%%%%%%%%%%%

\romain{Some remarks are given next:
\begin{itemize}
    \item We can state Theorem \ref{thm-scaling-optimal-value-function} with $V_{d,\gamma_1,\gamma_2}(x)$ for some $\gamma_1\in\Rlp$ and $\gamma_2\in\R$ instead of $V_{d,1,1}(x)$. This may be useful for stabilization purposes, as we may balance the effect of the weight $\varepsilon^{-\mu\nu^{k}}$ on a given compact set..
    \item The cost we obtain in (\ref{eq-thm-scaling-optimal-value-function}) is discounted or reversely discounted in different way compared to what we are used to. This form does not allow us to write a nice Bellman equation as in the classical (reversely) discounted case, but we may still be able to exploit it to analyse stability.
    \item If we want to exploit (\ref{eq-thm-scaling-optimal-value-function}) to derive stabilizing sequence of inputs applied in a receding horizon fashion, we would have to be careful as, at each instant, the applied control input would be the first element of a sequence of optimal inputs for a different cost. However, our usual assumptions are uniform, so we might be able to cope with it.
    \item If we can obtain a satisfying stabilization result based on Theorem \ref{thm-scaling-optimal-value-function}, it would be interesting to explicitly address the sampling of the unit sphere on which optimal control inputs would be computed. This result would also be new in the case where $\nu=1$ as this is not  addressed in \cite{Grimm-et-al-tac2005}. This might for instance be useful for switched linear systems I feel as I guess SA\ref{sass-homogeneity-f} will hold with $\nu=1$. We would have to restrict the class of stage costs but still. 
    \item It would be nice to include input constraints. This is done for instance in \cite[item 3) of Proposition 1]{Grimm-et-al-tac2005}.
            \item Dragan feels we should investigate more the relationships between continuous-time and discrete-time homogeneity notions. Looking  sampled-data systems with fast sampling may help to clarify this. The authors of \cite{Sanchez-et-al-ijrnc19} have investigated discretization issues in their more recent works. It would be good to look at these.
            \item It would be interesting to study a stochastic version of the above results and see  whether a probabilistic notion of homogeneity might be more suitable/needed in this case.
\item A general comment: the homogeneity notion we consider relies on dilations with the respect to the origin, and necessarily $f(0,0)=0$. Since we may be interested in set stability, I am wondering whether it would make sense to consider dilations with respect to a set. I have never seen such a notion, but we might think about it.
    \item Another general comment: the notion of homogeneity proposed in \cite{Sanchez-et-al-ijrnc19} might be useful to study homogeneous hybrid systems. This is totally unrelated to optimal control, but we may keep this in our mind for the future.
\end{itemize}}



